Protoplanetary Disk Polarization at Multiple Wavelengths: Are Dust Populations Diverse?

Millimeter and sub-millimeter observations of continuum linear dust polarization provide insight into dust grain growth in protoplanetary disks, which are the progenitors of planetary systems. We present the results of the first survey of dust polarization in protoplanetary disks at 870 $\mu$m and 3 mm. We find that protoplanetary disks in the same molecular cloud at similar evolutionary stages can exhibit different correlations between observing wavelength and polarization morphology and fraction. We explore possible origins for these differences in polarization, including differences in dust populations and protostar properties. For RY Tau and MWC 480, which are consistent with scattering at both wavelengths, we present models of the scattering polarization from several dust grain size distributions. These models aim to reproduce two features of the observational results for these disks: (1) both disks have an observable degree of polarization at both wavelengths and (2) the polarization fraction is higher at 3 mm than at 870 $\mu$m in the centers of the disks. For both disks, these features can be reproduced by a power-law distribution of spherical dust grains with a maximum radius of 200 $\mu$m and high optical depth. In MWC 480, we can also reproduce features (1) and (2) with a model containing large grains ($a_{max}$ = 490 $\mu$m ) near the disk midplane and small grains ($a_{max}$ = 140 $\mu$m) above and below the midplane.

==> pol_spectra.tex <==
\subsection{Polarization spectra}
\label{sec:spectra}

The disks in this survey exhibit clear differences in the correlation between polarization morphology and observing wavelength. This may indicate differences in the disks' dust grain sizes or dust optical depths, or it could arise from differences in protostar luminosities. {\bf In this section, we examine each of these cases.} 

\citet{2022MNRAS.512.3922L} found that the transition between the azimuthal polarization morphology seen in sources such as HL Tau, DG Tau, and Haro 6-13 at 3 mm (which likely arises from dichroic emission of aligned grains) and the scattering polarization seen at 870 $\mu$m in the same source could be explained by optical depth effects. Optical depth influences which polarization mechanism dominates the polarized emission produced at a given wavelength. At low optical depths, the probability that a photon will encounter a dust grain and scatter to produce polarization are low. Therefore, the scattering polarization tends to be weaker than any polarization from direct thermal emission from aligned dust grains. At high optical depths, photons are likely to encounter an aligned dust grain, which preferentially absorb light whose E-vector is along their long axes. This preferential absorption, known as dichroic extinction, reduces the amount of polarized emission from thermal emission from aligned grains. On the other hand, high optical depths mean that a photon is likely to encounter a dust grain and scatter, thus raising the amount of scattering polarization. The scattering polarization at high optical depths is the net result of multiple scattering events. 

While the transition between azimuthal and scattering polarization occurs between 3 mm and 870 $\mu$m in Haro 6-13 and V892 Tau, RY Tau and MWC 480 are still both consistent with scattering at 3 mm. Given the relationship between polarization morphology and optical depth described in \citet{2022MNRAS.512.3922L}, we expect that if there are aligned grains in RY Tau and MWC 480, the transition between thermal and scattering polarization occurs at wavelengths longer than 3 mm. \sout{The differences in the sources' polarization spectra could be rooted in differences in their dust populations or differences in protostellar radiation properties.} Compared to Haro 6-13, RY Tau and MWC 480 also have brighter disks, which are likely to have  higher optical depths and thus a stronger scattering at 3 mm. V892 Tau's disk is brighter still, but its dust polarization may be affected by a large hole surrounding the binary system. It is {\bf also} interesting to note that RY Tau and MWC 480 have stellar masses significantly higher than that of Haro 6-13 ($\sim$2$M_\odot$ vs $\sim$1$M_\odot$). 

{\bf Another} possible reason for the differences in polarization morphology between the disks is that Haro 6-13 and V892 Tau do not contain dust grains large enough to efficiently create scattering polarization at 3 mm, or that the population of large dust grains in these sources is optically thin. We speculate that RY Tau and MWC 480 may have higher optical depths than Haro 6-13 due to their polarization spectra. If the transition between scattering and the azimuthal polarization pattern is controlled by optical depth, as explored in \citet{2022MNRAS.512.3922L}, then disks with higher optical depths would transition from showing polarization consistent with scattering to showing azimuthal polarization at longer wavelengths. Observing these disks in polarization at wavelengths longer than 3 mm would allow us to determine where the change in polarization morphology occurs in RY Tau and MWC 480. 

{\bf As described in \citet{2022FrASS...9.3927T}, the radiative alignment torque acting on a grain is directly proportionate to the energy density of the radiaton field.  A more luminous protostar would therefore create a stronger RAT, leading to a higher probability of radiatively-aligned grains.} {\bf V892 Tau is the most luminous source in our sample (see Table \ref{tab:disk_params}), and shows a transition between an azimuthal polarization morphology at 3 mm and a morphology consistent with scattering at 870 $\mu$m. RY Tau and MWC 480 are more luminous than Haro 6-13, but are consistent with scattering at both wavelengths, while Haro 6-13 shows the same transition of polarization morphologies as V892 Tau. All else being equal, we would expect higher protostar luminosities to lead to more polarization from radiative alignment, but other differences between the systems may have more influence on their polarization morphologies.} DL Tau's disk is less bright than RY Tau and MWC 480's, and it's protostar's luminosity is {\bf 0.65$L_\odot$}. DL Tau's polarization morphology cannot be conclusively determined from the tentative detection of polarization at 3 mm, since the polarized region was smaller than a beam, allowing for only one measurement of the polarization fraction and angle. If the polarized emission at 3 mm is real, then DL Tau's polarization spectrum resembles RY Tau and MWC 480's. However, higher sensitivity observations are needed to determine whether DL Tau has more extended polarized emission at 3 mm. Determining whether stellar mass and luminosity are correlated with polarization spectrum will require multi-wavelength polarization observations of a wider sample of disks.
